Elucidating the Design Space of Multimodal Protein Language Models

Multimodal protein language models (PLMs) integrate sequence and token-based structural information, serving as a powerful foundation for protein modeling, generation, and design. However, the reliance on tokenizing 3D structures into discrete tokens causes substantial loss of fidelity about fine-grained structural details and correlations. In this paper, we systematically elucidate the design space of multimodal PLMs to overcome their limitations. We identify tokenization loss and inaccurate structure token predictions by the PLMs as major bottlenecks. To address these, our proposed design space covers improved generative modeling, structure-aware architectures and representation learning, and data exploration. Our advancements approach finer-grained supervision, demonstrating that token-based multimodal PLMs can achieve robust structural modeling. The effective design methods dramatically improve the structure generation diversity, and notably, folding abilities of our 650M model by reducing the RMSD from 5.52 to 2.36 on PDB testset, even outperforming 3B baselines and on par with the specialized folding models. Project page and code: https://bytedance.github.io/dplm/dplm-2.1/.

==> figText/figure_template.tex <==
\begin{figure}[ht]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{fig/icml_numpapers.pdfhttps://bytedance.larkoffice.com/docx/JQosdEYcto4dn6x63yccTXOCnNh}}
\caption{Historical locations and number of accepted papers for International
Machine Learning Conferences (ICML 1993 -- ICML 2008) and International
Workshops on Machine Learning (ML 1988 -- ML 1992). At the time this figure was
produced, the number of accepted papers for ICML 2008 was unknown and instead
estimated.}
\label{icml-historical}
\end{center}
\vskip -0.2in
\end{figure}

==> figText/geometry_folding_over_time.tex <==
\begin{figure}[ht]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{fig/geometry_folding_over_time.pdf}}
\caption{\textbf{Effects of geometric designs on folding over training time.}}
\label{icml-historical}
\end{center}
\vskip -0.2in
\end{figure}

==> figText/multi_layer_ensemble_weight.tex <==
\begin{figure}[ht]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{fig/geometry_performance_efficiency_tradeoff.pdf}}
\caption{\textbf{Layer weight distribution in representation alignment.}}
\label{icml-historical}
\end{center}
\vskip -0.2in
\end{figure}

==> figText/summary_table.tex <==
\begin{figure}[h]
% \vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=1.0\columnwidth]{fig/Desing_Choice_Summary_Table.pdf}}
% \caption{\textbf{Case study of residual diffusion.} We visualize the difference between the PLM generated structure and residual diffusion refined structure. The gray and blue structure correspond to the PLM prediction and the residual diffusion-refined one, respectively. }
\label{fig:summary_table}
\end{center}
% \vskip -0.2in
\end{figure}

==> sec/4_1_geometric_module_and_signals.tex <==
\section{Improved Geometry-aware Architecture with Representation Alignment}
\label{sec:geo_dplm}


% 
As evidenced in protein folding~\cite{alphafold2,esm2}, the intricate nature of protein structures demands methods that capture higher-order relationship between residues beyond simple sequence-based models. While bit labels and flow matching effective guide the design of supervision targets, they lack the inductive biases that might be needed to capture the complexity of residual interactions. To address this limitation, we introduce \textit{geometric modules} and \textit{representation alignment} (\textit{REPA})~\cite{REPA} to enhance the understanding of residue-residue interactions and structural diversity. 

\textit{Geometric modules}~\cite{alphafold2} operates on compact 2D pair representations to capture pairwise spatial dependencies of residues. As shown in~\cref{fig:geometry_module}, we use a structure attention to independently refine structure representations and pair representations through transition and triangle layers, followed by the Seqstruct attention to integrate pair representations with both sequence and structural signals. 
We adopt \textit{REPA} by aligning the representations of the protein language model to transfer meaningful structural semantics from specialized folding model, ESMFold~\cite{esm2}. Originally successful in vision tasks, we find that REPA effectively improve the structural diversity of generated proteins by introducing additional learning signals. The effectiveness of these innovations are demonstrated in improved structure diversity (\cref{sec:generation-diversity}). We provide ablation study and efficiency analysis of geometric modules in \cref{sec:geometry-module}, and analyze the alignment setup of REPA in \cref{sec:repa}.

\input{figText/geometry_module}
\input{figText/geometry_module_detail}

\input{table/geometry_module}


\subsection{Analysis of Geometric Designs}
\label{sec:geometry-module}
In subsequence experiments, we use 16 H100s train each model for 100k steps using the 220K training data from PDB~\cite{PDB} and Swissprot~\cite{AFDB}, following the setting in DPLM-2~\cite{dplm2}. 

\paragraph{Component-wise analysis on structure folding.}
\cref{tab:ablation-geometry} provides a component-wise study on each geometry-based module, which could be referred in \cref{fig:struct_attn,fig:seqstruct_attn}. Introducing 2D pair representation maps into DPLM-2 effectively improves structure prediction, reducing the folding RMSD from 7.703 to 7.244 RMSD and increases the TMscore to 0.8339. When models are trained without the folding SFT objective $\max_\theta\log p_\theta(x|s)$, the inclusion of transition layers for structure representations proves critical for achieving better structure predictions. SeqStruct attention, which combines pair representations with sequence information, achieves minimal improvement in metrics, indicating that solely incoporating pair information into structure representations is sufficient. In contrast to the common practice in structure folding, we find that triangle update and attention operations do not yeild notable benefits. For simplicity, in subsequent experiments, we refer to the model with logits bias and pair representation transition layers as GeoDPLM.


\paragraph{Training efficiency of geometric designs.}
\cref{fig:geometry_efficiency} presents the correlation between training speed and structure prediction performance on Cameo2022 for each ablation variation in \cref{tab:ablation-geometry}. We report the average training speed every 10k training steps, and use marker colors to reflect diversity. Among all operations, triangle operations are the most computationally intensive, with triangle update (TU) and attention (TA) dramatically reducing the training efficiency by 3.9x and 6.8x, respectively. The attention mechanism involving pair representations as logits bias in GeoDPLM (Base) causes a slight decrease on training speed compared to DPLM2. Using transition layers for structure representations, which significantly boosts both structure modeling and generation diversity, has minimal impacts on training speed.

\input{figText/geometry_efficiency} 
% \input{figText/geometry_folding_over_time}


\subsection{Representation Alignments to Folding Model}
\label{sec:repa}
Applying REPA with folding models refines generation process and significantly increases generation diversity as shown in \cref{fig:generation-diversity}. In this section, we further discuss the setup of REPA and its effectiveness on structure prediction. 

\textbf{REPA setup.} We select ESMFold~\cite{esm2} as the target representation encoder due to its computational efficiency and open-source availability compared to other folding models~\cite{alphafold2,deepmind2023AF3}. Using the protein sequences in our training data, we precompute the structure and pair representations from the folding trunk of ESMFold. We run three recycling iterations within the folding trunk to ensure the quality of representations. Instead of aligning embeddings from a certain layer as done in~\citet{REPA}, we apply a learnable \texttt{nn.Parameter} followed by a softmax function as the weight to ensemble representations across all layers. We follow~\citet{REPA} to apply a 3-layer MLP to project the representations before aligning them with the target representations through negative cosine similarity.

\input{table/repa}
\textbf{Compatibility with different architectures.}
\cref{tab:repa} presents the effects of REPA on structure prediction. REPA improves structure folding on both PDB date split and Cameo datasets, highlighting its ability to go beyond refining the generation process. Importantly, we observe that REPA is versatile, being compatible with both language model-based architectures (DPLM-2) and those incorporating geometric designs (GeoDPLM). Applying REPA on DPLM-2 effectively increases both folding RMSD and TM-score, suggesting that additional learning signals can play a critical role in improving architectures that lack geometric inductive biases.

% \textbf{Multi-layer ensemble vs. single layer alignment.}
% We compare the effect

% \input{table/multi_layer_ensemble}


% \input{figText/multi_layer_ensemble_weight}


\subsection{Generation Diversity}
\label{sec:generation-diversity}
Protein language models often suffer low diversity in generated structures~\cite{dplm2}, potentially due to the lack of inductive biases to capture high-order correlations. Despite the limitation, \cref{fig:generation-diversity} shows that appropriate geometric architecture designs (Geo-DPLM) could effectively improve the generation diversity. Aligning representations to structure folding model further significantly increase the diversity of generated structures, showcasing its effectiveness in refining generation process. For each protein length, we generate 40 samples and quantify the diversity by the number of clusters identified by FoldSeek~\cite{foldseek}, normalized by the number of generated samples.

\input{figText/geometry_diversity}

==> table/algorithm_template.tex <==
\begin{algorithm}[tb]
   \caption{Bubble Sort}
   \label{alg:example}
\begin{algorithmic}
   \STATE {\bfseries Input:} data $x_i$, size $m$
   \REPEAT
   \STATE Initialize $noChange = true$.
   \FOR{$i=1$ {\bfseries to} $m-1$}
   \IF{$x_i > x_{i+1}$}
   \STATE Swap $x_i$ and $x_{i+1}$
   \STATE $noChange = false$
   \ENDIF
   \ENDFOR
   \UNTIL{$noChange$ is $true$}
\end{algorithmic}
\end{algorithm}

==> table/multi_layer_ensemble.tex <==
% Single Column Table
\begin{table}[t]
\caption{\textbf{REPA: alignment in a single layer versus multiple layers.}}
\label{tab:repa-mle}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
% \resizebox{1.0\linewidth}{!}{%
\begin{tabular}{ccc}
\toprule
    \multirow{2}{*}{Alignment Depth}
    & \multicolumn{2}{c}{Cameo 2022} 
    \\
      \cmidrule(lr){2-3}
    % &
    & {\metric{RMSD}}$\downarrow$ & {\metric{TMscore}}$\uparrow$ \\
\midrule
    0
    & 6.873 & 0.784
    \\
    1
    & 6.498	& 0.790
    \\
    3
    & 6.112	& 0.799
    \\
    Multi-layer ensemble
    & 6.112	& 0.799
    \\
\bottomrule
\end{tabular}
% }
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}


==> table/multimer_finetune_esmfold.tex <==
% Single Column Table
\begin{table}[t]
\caption{\textbf{Fine-tuning with multimer and monomer data.} We evaluate the effects of fine-tuning with PDB-Multimer and Swissprot on structure prediction. Incorporating multimer data improves both monomer and multimer folding. SFT: supervised fine-tuning with folding objective.}
\label{tab:multimer-co-train}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\resizebox{1.0\linewidth}{!}{%
\begin{tabular}{cccccccc}
\toprule
    \multirow{2}{*}{Method}
    &
    \multicolumn{2}{c}{Training Data} 
    & \multirow{2}{*}{SFT}
    & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}PDB\\-Multimer\end{tabular}} 
    & \multicolumn{2}{c}{Cameo 2022} 
    \\
    \cmidrule(lr){2-3} \cmidrule(lr){5-6} \cmidrule(lr){7-8}  
    % &
    & \begin{tabular}[c]{@{}c@{}}PDB\\-Multimer\end{tabular} & Swissprot & & {\metric{RMSD}}$\downarrow$ & {\metric{TMscore}}$\uparrow$ & {\metric{RMSD}}$\downarrow$ & {\metric{TMscore}}$\uparrow$ \\
\midrule
    ESMFold &
    - & - & -
    & 17.297 & 0.850
    & 3.899	 & 0.917
    \\
\midrule
    \multirow{4}{*}{DPLM-2} &
    & \greensurd &
    & 17.966 & 0.771
    & 7.703	 & 0.793
    \\
     &
    & \greensurd & \greensurd
    & 19.615 & \textbf{0.799}
    & 6.612	 & 0.823
    \\
     &
    \greensurd & & \greensurd
    & \textbf{16.146} & 0.775
    & 10.989 & 0.686
    \\
     &
    \greensurd & \greensurd & \greensurd
    & \underline{16.674} & \underline{0.798}
    & \textbf{6.410}	& \textbf{0.831}
    \\
\bottomrule
\end{tabular}
}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}


==> table/summary_table_old.tex <==
\begin{table}[htbp] % Use htbp for better placement flexibility
\caption{The taxonomy of design choices, their orthogonality, and a systematic synthesis of findings.}
\centering % Center the table environment

% --- Define column widths (adjust percentages as needed) ---
\newcommand{\colwidthA}{0.10\textwidth}
\newcommand{\colwidthB}{0.12\textwidth}
\newcommand{\colwidthC}{0.12\textwidth}
\newcommand{\colwidthD}{0.275\textwidth}
\newcommand{\colwidthE}{0.275\textwidth}

% --- Apply settings for this table only ---
{ % Start group to limit scope of \small and \arraystretch
% \small % Reduce font size (try \footnotesize if \small is not enough)
\footnotesize % Even smaller font size
\renewcommand{\arraystretch}{0.9} % Decrease row height slightly (default is 1.0)

\begin{tabular}{
    >{\columncolor[HTML]{FFFFFF}\raggedright\arraybackslash}m{\colwidthA} % Col 1
    >{\columncolor[HTML]{FFFFFF}\raggedright\arraybackslash}m{\colwidthB} % Col 2
    >{\columncolor[HTML]{FFFFFF}\raggedright\arraybackslash}m{\colwidthC} % Col 3
    >{\columncolor[HTML]{FFFFFF}\raggedright\arraybackslash}m{\colwidthD} % Col 4
    >{\columncolor[HTML]{FFFFFF}\raggedright\arraybackslash}m{\colwidthE}  % Col 5
}
\toprule
% ----- Header Row: Override default with centered alignment using \multicolumn -----
% Note: Using m{} columns centers vertically. For horizontal centering in headers, use \centering inside \multicolumn
\multicolumn{1}{>{\columncolor[HTML]{FFFFFF}\arraybackslash}m{\colwidthA}}{\small\color[HTML]{000000} \textbf{Design Space}} &
\multicolumn{1}{>{\columncolor[HTML]{FFFFFF}\centering\arraybackslash}m{\colwidthB}}{\small\color[HTML]{000000} \textbf{Design Choice}} & % Adjusted width reference to B
\multicolumn{1}{>{\columncolor[HTML]{FFFFFF}\centering\arraybackslash}m{\colwidthC}}{\small\color[HTML]{000000} \textbf{Traditional Choice}} &
\multicolumn{1}{>{\columncolor[HTML]{FFFFFF}\centering\arraybackslash}m{\colwidthD}}{\small\color[HTML]{000000} \textbf{Motivation}} &
\multicolumn{1}{>{\columncolor[HTML]{FFFFFF}\centering\arraybackslash}m{\colwidthE}}{\small\color[HTML]{000000} \textbf{Findings}} \\ \midrule

% --- Multirow Cell 1 ---
% For horizontal centering in multirow within a raggedright column, use a parbox
\multirow{6}[2]{=}{{Improved generative modeling}} & % Spans 3 logical groups, approx 6 physical lines potentially. Adjusted row count. Use \linewidth inside parbox.
% --- Other cells in these rows ---
  {\color[HTML]{000000} Bit-based modeling} &
  {\color[HTML]{000000} Index-based modeling} &
  {\color[HTML]{000000} Intuition: Small changes at the bit level can result in drastically different indices, making the learning process of index-based labels challenging. \par \vspace{0.5em} Empirical Analysis: Direct index prediction is highly inaccurate (8.64\% on Cameo).} & % Use \par instead of \newline\newline
  {\color[HTML]{000000} Bit-level supervision improves prediction accuracy across index and bit-level, while substantially reducing structural deviation from ground truth (RMSD and TMscore).} \\ \cmidrule{2-5}
  & {\color[HTML]{000000} ResDiff} &
  {\color[HTML]{000000} Decode tokens without residuals} &
  {\color[HTML]{000000} Quantizing continuous tokens into discrete ones amplifies reconstruction errors, suggesting that recovering the lost residuals might enhance structure prediction accuracy.} &
  {\color[HTML]{000000} ResDiff module performs fine-grained refinements on the local structure (Fig. 7), showing consistent performance improvements across different DPLM-2 variants.} \\ \cmidrule{2-5}
   & {\color[HTML]{000000}  Hybrid approach—data-space sampling and predicting discrete tokens } &
  {\color[HTML]{000000} Predict discrete tokens} &
  {\color[HTML]{000000} Discrete structure tokenization inevitably sacrifices atomic-level details.} &
  {\color[HTML]{000000} A hybrid approach with flow matching improves structure generation for the folding task and speeds up the sampling process by requiring 10x fewer sampling steps.} \\ \cmidrule{1-5} % Rule spans all columns

% --- Multirow Cell 2 ---
\multirow{4}{=}{Structure-aware \newline approaches} & % Spans 2 logical groups, approx 4+ physical lines. Adjusted row count.
% --- Other cells in these rows ---
  {\color[HTML]{000000} Geometry-aware architecture} &
  {\color[HTML]{000000} Sequence-based transformer architecture} &
  {\color[HTML]{000000} Protein structures require capturing higher-order relationships between residues, as evidenced in folding.} &
  {\color[HTML]{000000} Geometric modules enhance structure folding performance and generation diversity. Unlike typical folding models, our analysis shows that triangle layers provide little benefit while greatly slowing down training.} \\ \cmidrule{2-5}
  & {\color[HTML]{000000} Representation alignments to folding model} &
  {\color[HTML]{000000} Discrete token supervision only} &
  {\color[HTML]{000000} Discrete token supervision might be less effective for capturing finer atom-level details. Unlike discrete supervision that enforces strict and sharp targets, representation alignment enables smooth, informative and high-dimensional learning, preserving finer structural nuances and improving generation diversity.} &
  {\color[HTML]{000000} \vspace{0.2em}Representation alignment~\cite{REPA} considerably boosts generation diversity and is compatible with both language model-based and geometric architectures.
  \par % Separate paragraph for the list
  % Removed \vspace before list
  \vspace{0.5em}
  Alternative approaches: % Optional introductory text
    \begin{enumerate}[label=\arabic*., % Numbering style
                     leftmargin=1.5em,  % Indentation from left margin of cell
                     rightmargin=0pt, % No extra margin on the right
                     itemsep=0pt,    % Minimal space between items (was 0.2ex)
                     topsep=0pt,     % Minimal space above list (was 0.3ex)
                     partopsep=0pt,    % No extra space when list starts a paragraph
                     parsep=0pt]       % No extra space within item paragraphs
      \item Contact map supervision (esm2), quadratic complexity (L x L) resulting in extreme inefficiency in our prelim study
      \item Direct coordinate supervision: need to carefully take into account se3 symmetry. Recent progress on this: Proteina~\cite{proteina}.
      % \item % Your text for point 3 here (or remove \item if only 2 points)
    \end{enumerate}
  } \\ \midrule

% --- Row 6: Use default left alignment ---
{\color[HTML]{000000} Data} & % This doesn't need multirow, it's just one row category
  {\color[HTML]{000000} Multimer data exploration} &
  {\color[HTML]{000000} Monomer data only} &
  {\color[HTML]{000000} Multimer data presents diverse structural arrangements, while most existing PLMs are trained solely on monomer.} &
  {\color[HTML]{000000} Multimer and monomer modeling are deeply interconnected and leveraging multimer data advances structural modeling for both single and multi-chain proteins.} \\ \bottomrule
\end{tabular}
} % End group for \small and \arraystretch
\end{table}

==> table/table_template.tex <==
% Single Column Table
\begin{table}[t]
\caption{Classification accuracies for naive Bayes and flexible
Bayes on various data sets.}
\label{sample-table}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccr}
\toprule
Data set & Naive & Flexible & Better? \\
\midrule
Breast    & 95.9$\pm$ 0.2& 96.7$\pm$ 0.2& $\surd$ \\
Cleveland & 83.3$\pm$ 0.6& 80.0$\pm$ 0.6& $\times$\\
Glass2    & 61.9$\pm$ 1.4& 83.8$\pm$ 0.7& $\surd$ \\
Credit    & 74.8$\pm$ 0.5& 78.3$\pm$ 0.6&         \\
Horse     & 73.3$\pm$ 0.9& 69.7$\pm$ 1.0& $\times$\\
Meta      & 67.1$\pm$ 0.6& 76.5$\pm$ 0.5& $\surd$ \\
Pima      & 75.1$\pm$ 0.6& 73.9$\pm$ 0.5&         \\
Vehicle   & 44.9$\pm$ 0.6& 61.5$\pm$ 0.4& $\surd$ \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}


==> table/table_template_two_col.tex <==
\begin{table*}[t]
\caption{Classification accuracies for naive Bayes and flexible
Bayes on various data sets.}
\label{sample-table}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccr}
\toprule
Data set & Naive & Flexible & Better? \\
\midrule
Breast    & 95.9$\pm$ 0.2& 96.7$\pm$ 0.2& $\surd$ \\
Cleveland & 83.3$\pm$ 0.6& 80.0$\pm$ 0.6& $\times$\\
Glass2    & 61.9$\pm$ 1.4& 83.8$\pm$ 0.7& $\surd$ \\
Credit    & 74.8$\pm$ 0.5& 78.3$\pm$ 0.6&         \\
Horse     & 73.3$\pm$ 0.9& 69.7$\pm$ 1.0& $\times$\\
Meta      & 67.1$\pm$ 0.6& 76.5$\pm$ 0.5& $\surd$ \\
Pima      & 75.1$\pm$ 0.6& 73.9$\pm$ 0.5&         \\
Vehicle   & 44.9$\pm$ 0.6& 61.5$\pm$ 0.4& $\surd$ \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}
